Cross-correlation Weak Lensing of SDSS Galaxy Clusters I: Measurements

This is the first in a series of papers on the weak lensing effect caused by clusters of galaxies in Sloan Digital Sky Survey. The photometrically selected cluster sample, known as MaxBCG, includes ~130,000 objects between redshift 0.1 and 0.3, ranging in size from small groups to massive clusters. We split the clusters into bins of richness and luminosity and stack the surface density contrast to produce mean radial profiles. The mean profiles are detected over a range of scales, from the inner halo (25 kpc/h) well into the surrounding large scale structure (30 Mpc/h), with a significance of 15 to 20 in each bin. The signal over this large range of scales is best interpreted in terms of the cluster-mass cross-correlation function. We pay careful attention to sources of systematic error, correcting for them where possible. The resulting signals are calibrated to the ~10% level, with the dominant remaining uncertainty being the redshift distribution of the background sources. We find that the profiles scale strongly with richness and luminosity. We find the signal within a given richness bin depends upon luminosity, suggesting that luminosity is more closely correlated with mass than galaxy counts. We split the samples by redshift but detect no significant evolution. The profiles are not well described by power laws. In a subsequent series of papers we invert the profiles to three-dimensional mass profiles, show that they are well fit by a halo model description, measure mass-to-light ratios and provide a cosmological interpretation.

==> Makefile <==
TEXFILE=maxbcg_lensing
default: dvi

# just run it
bib: 
	bibtex ${TEXFILE}

dvi: 
	latex ${TEXFILE}
	latex ${TEXFILE}

ps: 
	dvips -t letter ${TEXFILE} -o ${TEXFILE}.ps

pdf:
	latex ${TEXFILE}
	latex ${TEXFILE}
	dvipdfm ${TEXFILE}.dvi #${TEXFILE}.pdf

# Remember to go ahead and make inside the astro-ph directory because
# they don't run bibtex
dir=${TEXFILE}_astro_ph
aph:
	rm -rf ${dir}
	rm -f ${dir}.tar.gz
	mkdir ${dir}
	mkdir ${dir}/plots
	cp maxbcg_lensing.bbl ${dir}/
	cp *.tex ${dir}/
	cp *.cls ${dir}/
	cp plots/*.eps ${dir}/plots/
	cp Makefile ${dir}/
tar:
	rm -f ${dir}.tar.gz
	tar cvfz ${dir}.tar.gz ${dir}

clean:
	rm \
	${TEXFILE}.dvi \
	${TEXFILE}.ps \
	${TEXFILE}.pdf \
	${TEXFILE}.aux \
	${TEXFILE}.bbl \
	${TEXFILE}.blg \
	${TEXFILE}.log 





==> maxbcg_authorlist.tex <==
\author{
Erin S. Sheldon,\altaffilmark{1}
David E. Johnston,\altaffilmark{2,3}
Ryan Scranton,\altaffilmark{4}
Ben Koester,\altaffilmark{5}
Timothy A. McKay,\altaffilmark{5}
Hiroaki Oyaizu,\altaffilmark{6,7}
Carlos Cunha,\altaffilmark{6,7}
Marcos Lima,\altaffilmark{7,8}
Huan Lin,\altaffilmark{9}
Joshua A. Frieman,\altaffilmark{6,7,9}
Risa Wechsler,\altaffilmark{7}
James Annis,\altaffilmark{9}
Rachel Mandelbaum,\altaffilmark{10}
Neta A. Bahcall,\altaffilmark{11}
and Masataka Fukugita\altaffilmark{12}
}

\altaffiltext{1}{Department of Physics, New York University, 4 Washington Place, New York, NY 10003.}
\altaffiltext{2}{Department of Astronomy, 105-24, California Institute of Technology, 1201 East California Boulevard, Pasadena, CA 91125.}
\altaffiltext{3}{Jet Propulsion Laboratory 4800 Oak Grove Drive, Pasadena ,CA, 91109}
\altaffiltext{4}{Department of Physics and Astronomy, University of Pittsburgh, 3941 O'Hara Street, Pittsburgh, PA 15260.}
\altaffiltext{5}{Department of Physics, University of Michigan, 500 East University, Ann Arbor, MI 48109-1120.}
\altaffiltext{6}{Department of Astronomy and Astrophysics, The University of Chicago, 5640 South Ellis Avenue, Chicago, IL 60637.}
\altaffiltext{7}{Kavli Institute for Cosmological Physics, The University of Chicago, 5640 South Ellis Avenue Chicago, IL  60637}
\altaffiltext{8}{Department of Physics, The University of Chicago, 5640  South Ellis Avenue, Chicago IL 60637}
\altaffiltext{9}{Fermi National Accelerator Laboratory, P.O. Box 500, Batavia, IL 60510.}
\altaffiltext{10}{Department of Physics, Jadwin Hall, Princeton University, Princeton, NJ 08544}
\altaffiltext{11}{Princeton University Observatory, Peyton Hall, Princeton, NJ 08544.}
\altaffiltext{12}{Institute for Cosmic Ray Research, University of Tokyo, 5-1-5 Kashiwa, Kashiwa City, Chiba 277-8582, Japan.}

